Street-Level AI: Are Large Language Models Ready for Real-World Judgments?

A surge of recent work explores the ethical and societal implications of large-scale AI models that make "moral" judgments. Much of this literature focuses either on alignment with human judgments through various thought experiments or on the group fairness implications of AI judgments. However, the most immediate and likely use of AI is to help or fully replace the so-called street-level bureaucrats, the individuals deciding to allocate scarce social resources or approve benefits. There is a rich history underlying how principles of local justice determine how society decides on prioritization mechanisms in such domains. In this paper, we examine how well LLM judgments align with human judgments, as well as with socially and politically determined vulnerability scoring systems currently used in the domain of homelessness resource allocation. Crucially, we use real data on those needing services (maintaining strict confidentiality by only using local large models) to perform our analyses. We find that LLM prioritizations are extremely inconsistent in several ways: internally on different runs, between different LLMs, and between LLMs and the vulnerability scoring systems. At the same time, LLMs demonstrate qualitative consistency with lay human judgments in pairwise testing. Findings call into question the readiness of current generation AI systems for naive integration in high-stakes societal decision-making.

==> tables/llm_conditions.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Experiment \\ Type\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Vignette\\ Provided\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Outcome Prediction\\ Provided\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Task: First\\ Predict Outcome\end{tabular}} \\ \hline
Blind Start & \tick & \cross & \cross \\
Vision Only & \cross & \tick & \cross \\
Shared Vision & \tick & \tick & \cross \\
Vision First & \tick & \cross & \tick \\ \hline
\end{tabular}%
}
\caption{Experimental configurations used to prompt the LLM with different combinations of input and task.}
\label{table:llm_conditions}
\end{table}

==> tables/num_data_ranking_CI.tex <==

% \begin{table}[ht]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|ccc|ccc|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Score Type}}} & \multirow{2}{*}{\textbf{Dataset Name}} & \multirow{2}{*}{\textbf{Num Samples}} & \multicolumn{3}{c|}{\textbf{SPDAT}} & \multicolumn{3}{c|}{\textbf{RMFS}} \\ \cline{4-9} 
% \multicolumn{1}{|c|}{} &  &  & \multicolumn{1}{c|}{\textbf{Minimum Correlation}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Upper Bound} & \multicolumn{1}{c|}{\textbf{Minimum Correlation}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Upper Bound} \\ \hline
% \textbf{VISPDAT} & $VI_{SA}$ & 325 & \multicolumn{1}{c|}{0.98350} & \multicolumn{1}{c|}{0.97852} & 0.98733 & \multicolumn{1}{c|}{0.99360} & \multicolumn{1}{c|}{0.99165} & 0.99510 \\
% \textbf{VI-FSPDAT} & $VI_{F}$ & 698 & \multicolumn{1}{c|}{0.98419} & \multicolumn{1}{c|}{0.98107} & 0.98679 & \multicolumn{1}{c|}{0.99216} & \multicolumn{1}{c|}{0.99060} & 0.99346 \\
% \textbf{TAY-VISPDAT} & $VI_{Y}$ & 561 & \multicolumn{1}{c|}{0.98692} & \multicolumn{1}{c|}{0.98401} & 0.98930 & \multicolumn{1}{c|}{0.98853} & \multicolumn{1}{c|}{0.98598} & 0.99063 \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{table:ranking_num_data_CI}
% \end{table}



\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|cc|cc|}
\hline
\multirow{2}{*}{\textbf{Assessment Type}} & \multirow{2}{*}{\textbf{Dataset Name}} & \multirow{2}{*}{\textbf{Num Samples}} & \multicolumn{2}{c|}{\textbf{SPDAT}} & \multicolumn{2}{c|}{\textbf{RMFS}} \\ \cline{4-7} 
 &  &  & \multicolumn{1}{c|}{\textbf{Min Corr}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{Min Corr}} & \textbf{CI} \\ \hline
\textbf{VISPDAT} & $VI_{SA}$ & 325 & \multicolumn{1}{c|}{0.9835} & (0.97852, 0.98733) & \multicolumn{1}{c|}{0.9936} & (0.99165, 0.99510) \\
\textbf{VIFSPDAT} & $VI_{F}$ & 698 & \multicolumn{1}{c|}{0.98419} & (0.98107, 0.98679) & \multicolumn{1}{c|}{0.99216} & (0.99060, 0.99346) \\
\textbf{TAY} & $VI_{Y}$ & 561 & \multicolumn{1}{c|}{0.98692} & (0.98401, 0.98930) & \multicolumn{1}{c|}{0.98853} & (0.98598, 0.99063) \\ \hline
\end{tabular}%
}
\caption{Summary of each assessment type, its corresponding dataset name, and the number of samples used in the ranking task. The final two columns report the minimum Spearman’s $\rho$ observed over 10 independent random tie-break trials for the SPDAT, and RMFS induced rankings, respectively. All p-values for these correlations are effectively zero at ten significant figures.}
\label{labeltable:ranking_num_data_CI}
\end{table}

==> tables/robustness_spearman_CI.tex <==
% \begin{table}[ht]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|ccc|ccc}
% \hline
% \multirow{2}{*}{Assessment Type} & \multicolumn{3}{c|}{Between LLAMA Rankings} & \multicolumn{3}{c}{Between DeepSeek Rankings} \\ \cline{2-7} 
%  & \multicolumn{1}{c|}{$\rho$} & \multicolumn{1}{c|}{Lower Bound} & Upper Bound & \multicolumn{1}{c|}{$\rho$} & \multicolumn{1}{c|}{Lower Bound} & \multicolumn{1}{c|}{Upper Bound} \\ \hline
% $VI_{SA}$ & \multicolumn{1}{c|}{0.24692} & \multicolumn{1}{c|}{0.14032} & 0.34786 & \multicolumn{1}{c|}{0.47951} & \multicolumn{1}{c|}{0.38594} & \multicolumn{1}{c|}{0.56332} \\
% $VI_{F}$ & \multicolumn{1}{c|}{0.12805} & \multicolumn{1}{c|}{0.05405} & 0.20064 & \multicolumn{1}{c|}{0.27571} & \multicolumn{1}{c|}{0.20437} & \multicolumn{1}{c|}{0.34414} \\
% $VI_{Y}$ & \multicolumn{1}{c|}{0.19748} & \multicolumn{1}{c|}{0.11581} & 0.2765 & \multicolumn{1}{c|}{0.02719} & \multicolumn{1}{c|}{-0.05573} & \multicolumn{1}{c|}{0.10974} \\ \hline
% \end{tabular}%
% }
% \caption{Spearman Rank Correlations along with their 95\% confidence intervals between two different runs of the same LLM}
% \label{tab:robustness_spearman_CI}
% \end{table}




\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Assessment \\ Data\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Between LLAMA\\  Rankings\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Between DeepSeek\\  Rankings\end{tabular}}} \\ \cline{2-5} 
 & \multicolumn{1}{c|}{\textbf{$\rho$}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{$\rho$}} & \textbf{CI} \\ \hline
$VI_{SA}$ & \multicolumn{1}{c|}{0.24692} & (0.14032, 0.34786) & \multicolumn{1}{c|}{0.47951} & (0.38594, 0.56332) \\
$VI_{F}$ & \multicolumn{1}{c|}{0.12805} & (0.05405, 0.20064) & \multicolumn{1}{c|}{0.27571} & (0.20437, 0.34414) \\
$VI_{Y}$ & \multicolumn{1}{c|}{0.19748} & (0.11581, 0.27650) & \multicolumn{1}{c|}{0.02719} & (-0.05573, 0.10974) \\ \hline
\end{tabular}%
}
\caption{Spearman Rank Correlations along with their 95\% confidence intervals between two different runs of the same LLM}
\label{tab:robustness_spearman_CI}
\end{table}

==> tables/roc_table_closest_match.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[ht]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Assessment \\ Type\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# Positive\\ Samples\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Bureaucratic\\ Ranking\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RMFS\\ Ranking\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}LLaMA \\ Ranking 1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}LLaMA \\ Ranking 1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}DeepSeek \\ Ranking 1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}DeepSeek \\ Ranking 2\end{tabular}} \\ \hline
% \textbf{VISPDAT}                                                    & 45                                                                     & 0.77865                                                                 & 0.64357                                                         & 0.63389                                                             & 0.64651                                                             & 0.53389                                                                   & 0.50159                                                                   \\
% \textbf{VI-FSPDAT}                                                  & 12                                                                     & 0.5786                                                                  & 0.6578                                                          & 0.51543                                                             & 0.58297                                                             & 0.59524                                                                   & 0.65039                                                                   \\
% \textbf{TAY-VISPDAT}                                                & 8                                                                      & 0.58522                                                                 & 0.70389                                                         & 0.58635                                                             & 0.55199                                                             & 0.67495                                                                   & 0.55357                                                                   \\ \hline
% \end{tabular}%
% }
% \caption{ROC values by closest match to intervention by date}
% \label{tab:roc_closest_match}
% \end{table}




% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Assessment \\ Type\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# Positive\\ Samples\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Bureaucratic\\ Ranking\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RMFS\\ Ranking\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}LLaMA \\ Ranking 1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}LLaMA \\ Ranking 1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}DeepSeek \\ Ranking 1\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}DeepSeek \\ Ranking 2\end{tabular}} \\ \hline
\textbf{VISPDAT} & 64 & 0.69163 & 0.57962 & 0.6183 & 0.62482 & 0.52113 & 0.51102 \\
\textbf{VI-FSPDAT} & 75 & 0.52657 & 0.57117 & 0.52721 & 0.54926 & 0.51474 & 0.55634 \\
\textbf{TAY-VISPDAT} & 90 & 0.51113 & 0.5661 & 0.50385 & 0.5489 & 0.53628 & 0.50849 \\ \hline
\end{tabular}%
}
\caption{ROC values by closest match to intervention by date}
\label{tab:roc_closest_match}
\end{table}

==> tables/roc_table_intensive_match_CI.tex <==

% \begin{table}[ht]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|ccc|}
% \hline
% \multirow{2}{*}{\textbf{Assessment Data}} & \multirow{2}{*}{\textbf{# Positive}} & \multicolumn{3}{c|}{\textbf{VI-SPDAT Ranking}} & \multicolumn{3}{c|}{\textbf{RMFS Ranking}} & \multicolumn{3}{c|}{\textbf{LLaMA Ranking 1}} & \multicolumn{3}{c|}{\textbf{LLaMA Ranking 2}} & \multicolumn{3}{c|}{\textbf{DeepSeek-R1 Ranking 1}} & \multicolumn{3}{c|}{\textbf{DeepSeek-R1 Ranking 1}} \\ \cline{3-20} 
%  &  & \multicolumn{1}{c|}{\textbf{AUC}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Higher Bound} & \multicolumn{1}{c|}{\textbf{AUC}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Higher Bound} & \multicolumn{1}{c|}{\textbf{AUC}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Higher Bound} & \multicolumn{1}{c|}{\textbf{AUC}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Higher Bound} & \multicolumn{1}{c|}{\textbf{AUC}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Higher Bound} & \multicolumn{1}{c|}{\textbf{AUC}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Higher Bound} \\ \hline
% $VI_{SA}$ & 68 & \multicolumn{1}{c|}{0.69404} & \multicolumn{1}{c|}{0.62449} & 0.76359 & \multicolumn{1}{c|}{0.59791} & \multicolumn{1}{c|}{0.52841} & 0.66740 & \multicolumn{1}{c|}{0.61667} & \multicolumn{1}{c|}{0.54023} & 0.69312 & \multicolumn{1}{c|}{0.62434} & \multicolumn{1}{c|}{0.54843} & 0.70026 & \multicolumn{1}{c|}{0.51957} & \multicolumn{1}{c|}{0.44263} & 0.59651 & \multicolumn{1}{c|}{0.51247} & \multicolumn{1}{c|}{0.43261} & 0.59234 \\
% $VI_{F}$ & 116 & \multicolumn{1}{c|}{0.52804} & \multicolumn{1}{c|}{0.47414} & 0.58193 & \multicolumn{1}{c|}{0.52422} & \multicolumn{1}{c|}{0.46678} & 0.58165 & \multicolumn{1}{c|}{0.51518} & \multicolumn{1}{c|}{0.45844} & 0.57192 & \multicolumn{1}{c|}{0.53740} & \multicolumn{1}{c|}{0.48256} & 0.59224 & \multicolumn{1}{c|}{0.51271} & \multicolumn{1}{c|}{0.45238} & 0.57304 & \multicolumn{1}{c|}{0.54361} & \multicolumn{1}{c|}{0.48757} & 0.59965 \\
% $VI_{Y}$ & 103 & \multicolumn{1}{c|}{0.51304} & \multicolumn{1}{c|}{0.45453} & 0.57154 & \multicolumn{1}{c|}{0.57135} & \multicolumn{1}{c|}{0.51352} & 0.62918 & \multicolumn{1}{c|}{0.51015} & \multicolumn{1}{c|}{0.44594} & 0.57437 & \multicolumn{1}{c|}{0.53258} & \multicolumn{1}{c|}{0.46859} & 0.59658 & \multicolumn{1}{c|}{0.54498} & \multicolumn{1}{c|}{0.48796} & 0.60201 & \multicolumn{1}{c|}{0.50854} & \multicolumn{1}{c|}{0.44528} & 0.57180 \\ \hline
% \end{tabular}%
% }
% \caption{ROC AUC values interventions matched by highest intensity along with their 95\% confidence intervals}
% \label{tab:roc_intensive_match_CI}
% \end{table}



\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|cc|cc|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Assessment \\ Data\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}# Positive\\ Samples\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}VI-SPDAT \\ Ranking\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}RMFS \\ Ranking\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LLaMA \\ Ranking 1\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LLaMA \\ Ranking 2\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DeepSeek-R1 \\ Ranking 1\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DeepSeek-R1 \\ Ranking 2\end{tabular}}} \\ \cline{3-14} 
 &  & \multicolumn{1}{c|}{\textbf{AUC}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{AUC}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{AUC}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{AUC}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{AUC}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{AUC}} & \textbf{CI} \\ \hline
$VI_{SA}$ & 68 & \multicolumn{1}{c|}{0.69404} & (0.62449, 0.76359) & \multicolumn{1}{c|}{0.59791} & (0.52841, 0.6674) & \multicolumn{1}{c|}{0.61667} & (0.54023, 0.69312) & \multicolumn{1}{c|}{0.62434} & (0.54843, 0.70026) & \multicolumn{1}{c|}{0.51957} & (0.44263, 0.59651) & \multicolumn{1}{c|}{0.51247} & (0.43261, 0.59234) \\
$VI_{F}$ & 116 & \multicolumn{1}{c|}{0.52804} & (0.47414, 0.58193) & \multicolumn{1}{c|}{0.52422} & (0.46678, 0.58165) & \multicolumn{1}{c|}{0.51518} & (0.45844, 0.57192) & \multicolumn{1}{c|}{0.53740} & (0.48256, 0.59224) & \multicolumn{1}{c|}{0.51271} & (0.45238, 0.57304) & \multicolumn{1}{c|}{0.54361} & (0.48757, 0.59965) \\
$VI_{Y}$ & 103 & \multicolumn{1}{c|}{0.51304} & (0.45453, 0.57154) & \multicolumn{1}{c|}{0.57135} & (0.51352, 0.62918) & \multicolumn{1}{c|}{0.51015} & (0.44594, 0.57437) & \multicolumn{1}{c|}{0.53258} & (0.46859, 0.59658) & \multicolumn{1}{c|}{0.54498} & (0.48796, 0.60201) & \multicolumn{1}{c|}{0.50854} & (0.44528, 0.57180) \\ \hline
\end{tabular}%
}
\caption{ROC AUC values interventions matched by highest intensity}
\label{tab:roc_intensive_match_CI}
\end{table}

==> tables/spearman_with_bureauractic_CI.tex <==

% \begin{table}[ht]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|ccc|ccc|ccc|ccc|}
% \hline
% \multirow{2}{*}{\textbf{Assessment Population}} & \multirow{2}{*}{\textbf{Ranking Criterion}} & \multicolumn{3}{c|}{\textbf{LLaMA Ranking 1}} & \multicolumn{3}{c|}{\textbf{LLaMA Ranking 2}} & \multicolumn{3}{c|}{\textbf{DeepSeek Ranking 1}} & \multicolumn{3}{c|}{\textbf{DeepSeek Ranking 2}} \\ \cline{3-14} 
%  &  & \multicolumn{1}{c|}{\textbf{$\rho$}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Upper Bound} & \multicolumn{1}{c|}{\textbf{$\rho$}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Upper Bound} & \multicolumn{1}{c|}{\textbf{$\rho$}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Upper Bound} & \multicolumn{1}{c|}{\textbf{$\rho$}} & \multicolumn{1}{c|}{\textbf{Lower Bound}} & \textbf{Upper Bound} \\ \hline
% \multirow{2}{*}{$VI_{SA}$} & \textbf{VI-SPDAT} & \multicolumn{1}{c|}{-0.18009} & \multicolumn{1}{c|}{-0.28414} & -0.07185 & \multicolumn{1}{c|}{-0.18640} & \multicolumn{1}{c|}{-0.29019} & -0.07828 & \multicolumn{1}{c|}{0.12056} & \multicolumn{1}{c|}{0.01152} & 0.22676 & \multicolumn{1}{c|}{0.07167} & \multicolumn{1}{c|}{-0.03756} & 0.17920 \\
%  & \textbf{RMFS} & \multicolumn{1}{c|}{-0.00952} & \multicolumn{1}{c|}{-0.11819} & 0.09938 & \multicolumn{1}{c|}{0.12469} & \multicolumn{1}{c|}{0.01569} & 0.23076 & \multicolumn{1}{c|}{0.16421} & \multicolumn{1}{c|}{0.05570} & 0.26889 & \multicolumn{1}{c|}{0.14639} & \multicolumn{1}{c|}{0.03762} & 0.25172 \\ \hline
% \multirow{2}{*}{$VI_{F}$} & \textbf{VI-SPDAT} & \multicolumn{1}{c|}{-0.06960} & \multicolumn{1}{c|}{-0.14316} & 0.00472 & \multicolumn{1}{c|}{-0.19930} & \multicolumn{1}{c|}{-0.27021} & -0.12625 & \multicolumn{1}{c|}{0.21722} & \multicolumn{1}{c|}{0.14450} & 0.28761 & \multicolumn{1}{c|}{0.17079} & \multicolumn{1}{c|}{0.09728} & 0.24244 \\
%  & \textbf{RMFS} & \multicolumn{1}{c|}{0.08557} & \multicolumn{1}{c|}{0.01130} & 0.15890 & \multicolumn{1}{c|}{-0.01491} & \multicolumn{1}{c|}{-0.08902} & 0.05937 & \multicolumn{1}{c|}{0.12232} & \multicolumn{1}{c|}{0.04827} & 0.19503 & \multicolumn{1}{c|}{0.08018} & \multicolumn{1}{c|}{0.00589} & 0.15359 \\ \hline
% \multirow{2}{*}{$VI_{Y}$} & \textbf{VI-SPDAT} & \multicolumn{1}{c|}{-0.15286} & \multicolumn{1}{c|}{-0.23316} & -0.07050 & \multicolumn{1}{c|}{-0.16309} & \multicolumn{1}{c|}{-0.24311} & -0.08086 & \multicolumn{1}{c|}{0.06188} & \multicolumn{1}{c|}{-0.02109} & 0.14400 & \multicolumn{1}{c|}{0.04425} & \multicolumn{1}{c|}{-0.03871} & 0.12661 \\
%  & \textbf{RMFS} & \multicolumn{1}{c|}{-0.01904} & \multicolumn{1}{c|}{-0.10167} & 0.06385 & \multicolumn{1}{c|}{-0.02552} & \multicolumn{1}{c|}{-0.10809} & 0.05740 & \multicolumn{1}{c|}{0.06974} & \multicolumn{1}{c|}{-0.01322} & 0.15174 & \multicolumn{1}{c|}{0.02503} & \multicolumn{1}{c|}{-0.05788} & 0.10760 \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{tab:rank_correlations_CI}
% \end{table}



\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Assessment\\  Subpopulation\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Ranking \\ Criterion\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LLaMA \\ Ranking 1\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LLaMA \\ Ranking 2\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DeepSeek \\ Ranking 1\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DeepSeek \\ Ranking 2\end{tabular}}} \\ \cline{3-10} 
 &  & \multicolumn{1}{c|}{\textbf{$\rho$}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{$\rho$}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{$\rho$}} & \textbf{CI} & \multicolumn{1}{c|}{\textbf{$\rho$}} & \textbf{CI} \\ \hline
\multirow{2}{*}{$VI_{SA}$} & \textbf{VI-SPDAT} & \multicolumn{1}{c|}{-0.18009} & (-0.28414, -0.07185) & \multicolumn{1}{c|}{-0.18640} & (-0.29019, -0.07828) & \multicolumn{1}{c|}{0.12056} & (0.01152, 0.22676) & \multicolumn{1}{c|}{0.07167} & (-0.03756, 0.17920) \\
 & \textbf{RMFS} & \multicolumn{1}{c|}{-0.00952} & (-0.11819, 0.09938) & \multicolumn{1}{c|}{0.12469} & (0.01569, 0.23076) & \multicolumn{1}{c|}{0.16421} & (0.05570, 0.26889) & \multicolumn{1}{c|}{0.14639} & (0.03762, 0.25172) \\ \hline
\multirow{2}{*}{$VI_{F}$} & \textbf{VI-SPDAT} & \multicolumn{1}{c|}{-0.06960} & (-0.14316, 0.00472) & \multicolumn{1}{c|}{-0.19930} & (-0.27021, -0.12625) & \multicolumn{1}{c|}{0.21722} & (0.14450, 0.28761) & \multicolumn{1}{c|}{0.17079} & (0.09728, 0.24244) \\
 & \textbf{RMFS} & \multicolumn{1}{c|}{0.08557} & (0.01130, 0.15890) & \multicolumn{1}{c|}{-0.01491} & (-0.08902, 0.05937) & \multicolumn{1}{c|}{0.12232} & (0.04827, 0.19503) & \multicolumn{1}{c|}{0.08018} & (0.00589, 0.15359) \\ \hline
\multirow{2}{*}{$VI_{Y}$} & \textbf{VI-SPDAT} & \multicolumn{1}{c|}{-0.15286} & (-0.23316, -0.07050) & \multicolumn{1}{c|}{-0.16309} & (-0.24311, -0.08086) & \multicolumn{1}{c|}{0.06188} & (-0.02109, 0.14400) & \multicolumn{1}{c|}{0.04425} & (-0.03871, 0.12661) \\
 & \textbf{RMFS} & \multicolumn{1}{c|}{-0.01904} & (-0.10167, 0.06385) & \multicolumn{1}{c|}{-0.02552} & (-0.10809, 0.05740) & \multicolumn{1}{c|}{0.06974} & (-0.01322, 0.15174) & \multicolumn{1}{c|}{0.02503} & (-0.05788, 0.10760) \\ \hline
\end{tabular}%
}
\caption{Spearman Rank Correlations}
\label{tab:rank_correlations_CI}
\end{table}
